Learning to Generalize One Sample at a Time with Self-Supervision

Although deep networks have significantly increased the performance of visual recognition methods, it is still challenging to achieve the robustness across visual domains that is necessary for real-world applications. To tackle this issue, research on domain adaptation and generalization has flourished over the last decade. An important aspect to consider when assessing the work done in the literature so far is the amount of data annotation necessary for training each approach, both at the source and target level. In this paper we argue that the data annotation overload should be minimal, as it is costly. Hence, we propose to use self-supervised learning to achieve domain generalization and adaptation. We consider learning regularities from non annotated data as an auxiliary task, and cast the problem within an Auxiliary Learning principled framework. Moreover, we suggest to further exploit the ability to learn about visual domains from non annotated images by learning from target data while testing, as data are presented to the algorithm one sample at a time. Results on three different scenarios confirm the value of our approach.

==> experiments.tex <==
\paragraph{Datasets}
We test our model on the PACS \cite{hospedalesPACS} dataset for Domain Generalization and Unsupervised Domain adaptation benchmarks and on the CompCars \cite{Yang_2015_CVPR} and Portraits \cite{Ginosar_2015_ICCV_Workshops} datasets for Predictive Domain Adaptation experiments.

PACS is a recent but widely adopted test database for DG experiments, it is characterized by strong domain shifts between distributions, with both real images and artistic drawings. It contains approximately 10.000 images of 7 common categories across 4 different domains (Photo, Art painting, Cartoon, Sketch).

The Comprehensive Cars (CompCars) \cite{Yang_2015_CVPR} is a large-scale dataset composed of 136,726 vehicle photos taken in the space of 11 years (from 2004 to 2015). Follows the same experimental setting of \cite{massi} we select a subset of 24,151 images organized in 4 classes and 30 domains. The subset is composed by the images produced in the time range between 2009 and 2014 from 5 different view points. Considering the year of production and the perspective of the vehicle in the image we can identify 30 domains; the classes correspond to the type of vehicle (MPV, SUV, sedan and hatchback).

The Century of portraits (Portraits) \cite{Ginosar_2015_ICCV_Workshops} is a large set of pictures taken from American high school year-books. The photos cover a time range between 1905 and 2013 over 26 American states. Also in this case we follow \cite{massi} for the experimental protocol: we set a gender classification task performed on 40 domains obtained choosing 8 decades (from 1934) and 5 regions (New England, Mid Atlantic, Mid West, Pacific and Southern).



\paragraph{Self-supervised training}

We choose jigsaw puzzle solving as our self-supervised task. We treat each input as a 3x3 grid, scramble the tiles by randomly choosing one of 31 possible permutations, then train the $\auxblock$ module on the classification task of predicting which permutation was applied to the target image. Since no low level feature is available due to gradient propagation setting, the module is forced to recognize object parts and rearrange them with high level information alone. In our ablation studies, we also show experiments with the rotation task, in which we apply one out of four possible rotations, and train the network to predict the correct relative orientation.

The $\backbone$ module is trained on the main supervised task with unscrambled images, while the $\auxblock$ refines features of the original images for the main branch, but is only trained to rearrange scrambled images. For each training iteration, we feed the network mini-batches of scrambled and unscrambled images to train the auxiliary and main task respectively. We use batch accumulation to synchronously update weights of $\backbone$ and $\auxblock$, following the update rule shown in equation \ref{eq_update}

We find that setting the auxiliary loss weight to $\gamma = 2$ achieves training convergence for the auxiliary task, and leave it set at that value for all our experiments. It's also shown in the supplementary that changing this value has little to no effect on the final accuracy, as long as there is a stable convergence for the auxiliary task.

\paragraph{Experiments in Domain Generalization}

Our Domain Generalization experiments are run on the PACS dataset. We follow the experimental setting of \cite{hospedalesPACS}, using one domain as test and the others as sources, repeating the procedure until every domain has been used as the held out test and averaging cross-domain results.

To align our experiments with the training hyperparameters used in \cite{jigen}, we apply radom cropping, random horizontal flipping, photometric distortions and resize crops to 222x222 so that we get equally spaced square tiles on a 3x3 grid. Since we don't use domain annotations, all input images from source domains are randomly aggregated in mini-batches. We train the network for 40 epochs using SGD with momentum set at 0.9, an initial learning rate of 0.001, a cumulative batch size of 128 original images and 128 puzzles and a weight decay of 0.0005. We divide train inputs in 90\% train and 10\% validation splits, and test on the target with the best performing model on the validation set.


(Tables \ref{table:resultsDG_PACS}, \ref{table:resultsDG_officehome}, \ref{table:resultsDG_VLCS})
Note that with respect to \cite{hospedales19} we do not need to know a priori which is the source composition (number of domains and domain label for each source image). 

\paragraph{Adding the One-Shot Learning component}
After training with the aggregated sources, we fine-tune the $\auxblock$ module on puzzles of the incoming test sample following Algorithm 1. We keep all hyperparameters, including data augmentation strategy and auxiliary loss absolute magnitude, fixed to their initial training values and fine-tune the model for 3 iterations using a batch size of 128 scrambled images of the test sample. We revert back $\auxblock$ to the original weights when applying the procedure to a new sample.
%(Table \ref{table:analysisDG_PACS}).

\paragraph{Domain Generalization Results}

Table \ref{table:resultsDG_PACS} shows the result of \our (without fine-tuning) and \ourOS (after finetuning on test sample) algorithms on the PACS DG setting. We show that \our trained on the puzzle solving auxiliary task outperforms the JiGen algorithm and previous baselines except for the episodic training method of \cite{hospedales19}. When adding the finetuning component for 3 iterations, \ourOS improves average accuracy on every PACS target split and surpasses previous published results in this setting. Since also the JiGen algorithm uses auxiliary tasks, we add the target sample finetuning algorithm to \cite{jigen} and show that, although not as much as in \our, also JiGen improves from OS training.

To further demonstrate the effectiveness of the proposed methodology, we also create a fair baseline (null hypothesis) in which we train our entire model with the combine source algorithm without using auxiliary tasks and conditioned gradient propagation. Results in table \ref{table:resultsDG_PACS} shows that improvements are largely due to self-supervision and one-sample finetuning rather than increased depth or parameter count.

\paragraph{Extension to Unsupervised Domain Adaptation}

We run experiments on PACS on the Domain Adaptation setting proposed by \cite{jigen}. We use the same training hyperparameters used in Domain Generalization experiments, with the difference that we teach the self-supervised task using target images from the unlabeled domain only, and we validate the network on the puzzle task using and held-out split from the target. Even without using any explicit domain adaptation method, results in table \ref{table:resultsDA_PACS} shows that the model closes the representation gap with the target domain, yielding a $4.62$ accuracy increase over the combine source baseline. This supports our Domain Generalization results, showing that our architecture adapts to the unseen domain by solving puzzles on the target.

Although our DA results are inferior compared to the ones in \cite{jigen} and \cite{massi}, the latter all use the entropy loss for adaptation which, besides not being applicable to our Domain Generalization algorithm, needs to be tuned to be effective. We replicate experiments in \cite{jigen} and show in figure \ref{fig:ablation_jigsaw} that the JiGen algorithm is very sensitive to its hyperparameters, particularly the entropy loss weight, which dramatically drops performances if not tuned correctly.

\begin{figure}[tb]%\hspace{-5mm}
%\begin{tabular}{c@{~}c}
\centering
\includegraphics[height=4cm]{figures/BIG_jigenPACSablation-DA_full-crop.pdf}
%\end{tabular}the first (and unique) deep architecture de-
signed to tackle PDA: AdaGraph [52].  This method con-
sists in modeling the dependencies between the various do-
mains building a graph.  Each node denotes a domain and
the weight of each edge is a measure of how two domains
are connected.  This value is computed as a function of the
domain-specific metadata.  The method,  together with the
graph,  uses domain-specific batch-normalization layers to
extracts one model for each domain. Although this method
was created ad-hoc for a P
\caption{Analysis of JiGen in the PACS DA setting. The parameter $\gamma$ weights the 
entropy loss that involves the target data. Moreover the method exploits two different
source ($\alpha_s$) and target ($\alpha_t$) jigsaw loss weights.}
    \label{fig:ablation_jigsaw}%\vspace{-3mm}
\end{figure}

\begin{table}[tb]
\begin{center} \small
\begin{tabular}{@{}c@{}c@{}c@{~~}c@{~~}c@{~~}c|@{~~}c}
\hline
\multicolumn{2}{@{}c@{}}{\textbf{PACS-DA}}  & \textbf{art\_paint.} & \textbf{cartoon} &  \textbf{sketches} & \textbf{photo} &   \textbf{Avg.}\\ \hline
% 
\multicolumn{7}{@{}c@{}}{\textbf{Resnet-18}}\\
\hline
\multirow{3}{*}{\cite{mancini2018boosting}}& Deep All & 74.70 & 72.40 & 60.10 & 92.90 & 75.03\\
& Dial & 87.30 & 85.50 & 66.80 & 97.00 &  84.15 \\
& DDiscovery  &  \textbf{87.70}	& \textbf{86.90}	& 69.60 & 97.00		& 85.30\\
\hline
\multirow{2}{*}{\cite{jigen}}& Deep All & 77.85  & 74.86  & 67.74  & 95.73  & 79.05 \\
& JiGen &  84.88 &	81.07 &	\textbf{79.05} &	\textbf{97.96} &	\textbf{85.74} \\
%& JiGen $\gamma = 0$   &   &   &   &  &  \\
\hline
& \textbf{\our}    & 80.96  &  77.56 & 78.78  & 97.39 &  83.67\\
%& \textbf{Ro-Rock}    &   &   &   &  &  \\
%& \textbf{Ji-Ro-Rock}    &   &   &   &  &  \\
\hline
\end{tabular}
\caption{Multi-source Domain Adaptation results on PACS obtained as average over 3 repetitions for each run.}
\label{table:resultsDA_PACS}
\end{center}%\vspace{-8mm}
\end{table}

\paragraph{Extension to other self-supervised knowledge types: rotation}

As an ablation experiment, we run Domain Generalization experiments on the PACS dataset using rotation prediction as an auxiliary self-supervised task. We report in table (?) results of our method, with and without the fine-tuning step, which we run for 1 iteration only. Rotation is underperforming compared to jigsaw puzzle solving for PACS classification, with results inferior to the null hypothesis, revealing that the choice of self-supervision influences generalization capabilities. We still observe that, even when using the rotation auxiliary task, by running the finetuning step for just 1 iteration, the model is still able to adapt to the target sample and close the representation gap with refined information.

\paragraph{Extension to Predictive DA without metadata (is a DG setting)}
%Show thow JiGen, \our and \our+os work on the COMPCARS dataset.
Partial domain adaptation (PDA) \cite{multivariatereg} is characterized by a DG setting in which the system has to learn a model that works well through several unknown domains. Generally, the PDA setting includes the possibility to see a labeled source domain and a set of unlabeled auxiliary domains during training. A typical PDA approach exploits metadata extracted from the auxiliary domains (image timestamp, camera pose, etc.) to perform generalization. We demonstrate the effectiveness of our method that, even without the use of metadata, outperforms the state of the art in two datasets: the \textit{Comprehensive Cars} (CompCars) \cite{Yang_2015_CVPR} and the \textit{Century of portraits} (Portraits) \cite{Ginosar_2015_ICCV_Workshops}.\\

For both datasets we follow the experimental protocol described in \cite{massi}. For CompCars, we select a pair of domains to be respectively source and target and use the remaining 28 as auxiliary unlabeled data. Considering all possible pairs of sources and target we average results of 870 experiments. A similar setting is applied for Portraits, for which we consider the \textit{across decades} scenario (source and target domains selected from the same decade) and the \textit{across region} scenario (source and target from the same region). In total we run 440 experiments for Portraits.
\begin{comment}
The \textit{Comprehensive Cars} (CompCars) \cite{Yang_2015_CVPR} is a large-scale dataset composed of 136,726 vehicle photos taken in the space of 11 years (from 2004 to 2015). Follows the same experimental setting of \cite{massi} we select a subset of 24,151 images organized in 4 classes and 30 domains. The subset is composed by the images produced in the time range between 2009 and 2014 from 5 different view points. Considering the year of production and the perspective of the vehicle in the image we can identify 30 domains; the classes correspond to the type of vehicle (\textit{MPV}, \textit{SUV}, \textit{sedan} and \textit{hatchback}). In the PDA setting \cite{massi} one domain is selected as source, one as target and the remaining 28 as auxiliary then, considering each possible combination, this setting results in 870 experiments. \\


The \textit{Century of portraits} (Portraits) \cite{Ginosar_2015_ICCV_Workshops} is a large set of pictures taken from American high school year-books. The photos cover a time range between 1905 and 2013 over 26 American states. Also in this case we follow \cite{massi} for the experimental protocol: we set a gender classification task performed on 40 domains obtained choosing 8 decades (from 1934) and 5 regions (\textit{New England}, \textit{Mid Atlantic}, \textit{Mid West}, \textit{Pacific} and \textit{Southern}). For the experiments two scenarios were considered: \textit{across decades}, in which for source and target domains the same region is selected (leading to 280 experiments) and \textit{across regions}, considering the same decade for source and target domains (160 experiments).\\
\end{comment}
As stated before, we don't use any metadata from auxiliary domains during training; the only way in which we exploit the auxiliary datasets is through the self-supervised task. To validate the strength of our approach we compared ourselves with the first (and unique) deep architecture designed to tackle PDA: AdaGraph \cite{massi}. This method consists in modeling the dependencies between the various domains building a graph. Each node denotes a domain and the weight of each edge is a measure of how much two domains are connected. This value is computed as a function of the domain-specific metadata. The method, together with the graph, uses domain-specific batch-normalization layers to extracts one model for each domain. Although this method was created ad-hoc for a PDA setting we show in Table \ref{table:resultsCOMPCARS} that \our outperforms AdaGraph in all settings. \\
Also in this set of experiments we use \our architecture implemented on ResNet-18 \cite{he2016deep} with the exact procedure and hyperparameters used in \cite{massi}. For the experiments on CompCars, starting with the network pretrained on ImageNet, we train for 6 epochs on source domain using Adam as optimizer with weight decay of $10^{6}$. The batch size used is 16 and the learning rate is $10^{-3}$ for the classifier and $10^{-4}$ for the rest of the network; the learning rate is decayed by a factor of 10 after 4 epochs. The jigsaw weight parameter was set to $2.0$. Also for the experiments on Portraits we use the same procedure and hyperparameters of \cite{massi} that are equal to that used for CompCars except for the number of epochs that in this case is 1 and for the jigsaw weight that in this case was set to $2.0$ for the experiments \textit{across decades} and to $1.0$ for the experiments \textit{across regions}.\\
Finally, also the \ourOS method has been tested in this setting and we noticed that the one-shot technque, in this particular scenario, not provide any additional information. The motivation is that we have so many images from auxiliary domains that the method in itself generalize as best it can.



\begin{table}[tb]
    \begin{center} \small
        \begin{tabular}{@{}c@{}c@{}c@{~}c@{~~~}c@{~~~}c|@{~~~}c}
        \hline
        \multicolumn{2}{c}{\textbf{PACS-DG}}  & \textbf{art\_paint.} & \textbf{cartoon} &  \textbf{sketches} & \textbf{photo} &   \textbf{Avg.}\\ \hline
        \multicolumn{7}{c}{\textbf{Resnet-18}}\\
        \hline
        & \hspace{-3mm} null hypothesis & 79.26  & 74.09  & 70.13  & 96.23  & 79.93 \\
        \hline
        & \textbf{\our}    & 78.95   &  74.36 & 73.99 & 96.29 &  80.90\\
        \hline
        & $\textbf{\ourOS}_{it=1}$   &  79.74  & 74.84  & 75.35  & 96.53 & 81.62 \\
        & $\textbf{\ourOS}_{it=2}$   & 79.79  & 75.01  & 76  & 96.61 & 81.85 \\
        & $\textbf{\ourOS}_{it=3}$   & 79.79  & 75.06  & 76  & 96.65 & 81.88 \\
        \hline
        & $\textbf{\our}_{rotations}$ & 79.49  & 74.11  & 70.6  & 95.87  & 79.52 \\
        & $\textbf{\ourOS}_{rotations}$   & 78.19  & 74.81  & 71.63  & 95.79 & 80.11 \\
        \hline
        \end{tabular}
        \caption{Final accuracy of \ourOS with increasing number of self-supervised iterations on the target sample}
        \label{table:resultsDG_PACS}
    \end{center}
\end{table}



\begin{table}[tb]
\begin{center} \small
\begin{tabular}{@{}c@{}c@{}c@{~}c@{~~~}c@{~~~}c|@{~~~}c}
\hline
\multicolumn{2}{c}{\textbf{PACS-DG}}  & \textbf{art\_paint.} & \textbf{cartoon} &  \textbf{sketches} & \textbf{photo} &   \textbf{Avg.}\\ \hline
\multicolumn{7}{c}{\textbf{Resnet-18}}\\
\hline
 \multirow{2}{*}{\cite{Antonio_GCPR18}} & Deep All & 77.87 & 75.89 & 69.27 &  95.19 & 79.55\\
 & D-SAM & 77.33 & 72.43 & 77.83 & 95.30 & 80.72\\
\hline
\multirow{4}{*}{\cite{hospedales19}}& Deep All & 77.60  & 73.90  & 70.30  & 94.40  & 79.10 \\
& DANN & 81.30  & 73.80  & 74.30  & 94.00  & 80.08 \\
& MLDG & 79.50  & 77.30  & 71.50  & 94.30  & 80.70 \\
& Reptile & 80.70  & 75.50  & 69.00  & 94.90  & 80.00 \\
& EPI-FCR & 82.10  & 77.00  & 73.00  & 93.90  & 81.50 \\
\hline
\multirow{3}{*}{\cite{jigen}} & Deep All & 77.85  & 74.86  & 67.74  & 95.73  & 79.05 \\
 & JiGen    & 79.4  & 75.25  & 71.35  &  96.03 &  80.51\\
 & JiGen \textbf{+ OS}   & 79.40  & 75.24  & 72.26  & 96.27  & 80.79 \\
 \hline
%& Deep All &   &   &   &   &  \\
 & \hspace{-3mm} null hypothesis & 79.26  & 74.09  & 70.13  & 96.23  & 79.93 \\
& \textbf{\our}    & 78.95   &  74.36 & 73.99 & 96.29 &  80.90\\
 & \textbf{\ourOS} & 79.79  & 75.06  & 76  & 96.65 & 81.88 \\

 \hline
%\end{tabular}
%\caption{Domain Generalization results on PACS. The results of \our are average over FIXME repetitions of each run. Each column title indicates the name of the domain used as target.}
%\label{table:resultsDG_PACS}
%\end{center}%\vspace{-8mm}
%\end{table}
%
%\begin{table}[tb]
%\begin{center} \small
%\begin{tabular}{@{}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c|@{~~~}c}
%\hline
%\multicolumn{2}{c}{\textbf{PACS}}  & \textbf{art\_paint.} & \textbf{cartoon} &  \textbf{sketches} & \textbf{photo} &   \textbf{Avg.}\\ \hline
%\multicolumn{7}{c}{\textbf{Resnet-18}}\\
%\end{tabular}
%\caption{Analysis on PACS}
%\label{table:analysisDG_PACS}
%\end{center}%\vspace{-8mm}
%\end{table}
%
%\begin{table}[tb]
%\begin{center} \small
%\begin{tabular}{@{}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c|@{~~~}c}
%\hline
%\multicolumn{2}{c}{\textbf{PACS}}  & \textbf{art\_paint.} & \textbf{cartoon} &  \textbf{sketches} & \textbf{photo} &   \textbf{Avg.}\\ \hline
%\multicolumn{7}{c}{\textbf{Resnet-18}}\\
\end{tabular}
%\caption{}
%\label{table:analysisDGROT_PACS}
\caption{Domain Generalization results on PACS. The results of \our are average over 3 repetitions of each run. Each column title indicates the name of the domain used as target.}
\label{table:resultsDG_PACS}
\end{center}%\vspace{-8mm}
\end{table}





\begin{table}[tb]
\begin{center} \small
\begin{tabular}{cccc}
\hline
Method & CompCars & Portraits-Dec. & Portraits-Reg.\\ \hline
Baseline & 56.8 & 82.3 & 89.2\\
AdaGraph & 58.8 & 87.0 & 91.0\\ \hline
%JiGen & 62.6 & &\\
\textbf{\our} & \textbf{60.2} & \textbf{87.1} & \textbf{91.6}\\
\textbf{\ourOS} & 60.0 & 87.1 & 91.5 \\
\hline
\end{tabular}
\caption{Results with ResNet-18 architecture.}
\label{table:resultsCOMPCARS}
\end{center}%\vspace{-8mm}
\end{table}

\begingroup
\begin{table}[tb]
\begin{center} \small
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{OS finetuning accuracy gains on individual \our instances} \\
\hline
target                       & instance     & \our      & OS 1 it.     & OS 2 it.    & OS 3 it.     \\
\hline
\multirow{3}{*}{photo}       & 1            & 96.41     & +0.12     & +0.18     & +0.30     \\
                             & 2            & 96.41     & +0.30     & +0.48     & +0.36     \\
                             & 3            & 96.05     & +0.30     & +0.30     & +0.42     \\
\hline
\multirow{3}{*}{art p.}      & 1            & 79.00     & +0.74     & +1.13     & +1.37     \\
                             & 2            & 78.71     & +0.83     & +0.33     & +0.09     \\
                             & 3            & 79.15     & +0.78     & +0.64     & +0.64     \\
\hline
\multirow{3}{*}{cartoon}     & 1            & 73.72     & +0.85     & +0.67     & +0.79     \\
                             & 2            & 74.23     & +0.17     & +0.34     & +0.39     \\
                             & 3            & 75.13     & +0,42     & +0.55     & +0.51     \\
\hline
\multirow{3}{*}{sketch}      & 1            & 73.45     & +1.53     & +2.04     & +2.04     \\
                             & 2            & 74.14     & +1.35     & +2.16     & +1.81     \\
                             & 3            & 74.37     & +1.20     & +1.83     & +2.19    \\
\hline
\end{tabular}
\caption{PACS DG experiments: accuracy gains of individual instances of \our when finetuned using OS with an increasing number of iterations. Results show the every model increases accuracy on the held-out test.}
\label{table:iterations}
\end{center}
\end{table}
\endgroup















\begin{comment}
\begin{table}[tbp]
\begin{center}\small
\begin{tabular}{@{}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c|c}
\hline
 \multicolumn{2}{c}{\textbf{Office-Home}}  & \textbf{Art} & \textbf{Clipart} &  \textbf{Product} & \textbf{Real-World} &  \textbf{Avg.}\\ \hline
\multicolumn{7}{c}{\textbf{Resnet-18}}\\
\hline
 \multirow{2}{*}{\cite{Antonio_GCPR18}} & Deep All  & 55.59 & 42.42 & 70.34 & 70.86 & 59.81 \\
 & D-SAM & \textbf{58.03} & 44.37 & 69.22 & 71.45 & 60.77\\
\hline
\multirow{2}{*}{\cite{jigen}} & Deep All & 52.15 & 45.86 &  70.86 & \textbf{73.15} & 60.51\\
 & JiGen & 53.04 & 47.51 & 71.47 & 72.79 & 61.20\\
\hline
& Deep All &   &   &   &   &  \\
& \textbf{\our}    &   &   &   &  &  \\
 & \textbf{\our + os}    &   &   &   &  &  \\
 \hline
\end{tabular}
\caption{Domain Generalization results on Office-Home. The results of \our are average over FIXME repetitions of each run. Each column title indicates the name of the domain used as target.}
\label{table:resultsDG_officehome}
\end{center}%\vspace{-6mm}
\end{table}

\begin{table}[tb]
\begin{center} \small
\begin{tabular}{@{}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c|c}
\hline
\multicolumn{2}{c}{\textbf{VLCS}}  & \textbf{Caltech} & \textbf{Labelme} &  \textbf{Pascal} & \textbf{Sun} &   \textbf{Avg.}\\ \hline
\multicolumn{7}{c}{\textbf{Resnet-18}}\\
\hline
% 
\multirow{3}{*}{[...]} & Deep All & 	& 	& 	& 	&   \\
& D-SAM & 	& 	& 	& 	& \\
& JiGen &   &   &   &   &  \\
\hline
& \textbf{\our}    &   &   &   &  &  \\
 & \textbf{\our + os}    &   &   &   &  &  \\
\hline
\end{tabular}
\caption{Domain Generalization results on VLCS. The results of \our are average over FIXME repetitions of each run. Each column title indicates the name of the domain used as target.}
\label{table:resultsDG_VLCS}%\vspace{-4mm}
\end{center}
\end{table}
\end{comment}

